Fast Propagation is Better: Accelerating Single-Step Adversarial Training via Sampling Subnetworks

Adversarial training has shown promise in building robust models against adversarial examples. A major drawback of adversarial training is the computational overhead introduced by the generation of adversarial examples. To overcome this limitation, adversarial training based on single-step attacks has been explored. Previous work improves the single-step adversarial training from different perspectives, e.g., sample initialization, loss regularization, and training strategy. Almost all of them treat the underlying model as a black box. In this work, we propose to exploit the interior building blocks of the model to improve efficiency. Specifically, we propose to dynamically sample lightweight subnetworks as a surrogate model during training. By doing this, both the forward and backward passes can be accelerated for efficient adversarial training. Besides, we provide theoretical analysis to show the model robustness can be improved by the single-step adversarial training with sampled subnetworks. Furthermore, we propose a novel sampling strategy where the sampling varies from layer to layer and from iteration to iteration. Compared with previous methods, our method not only reduces the training cost but also achieves better model robustness. Evaluations on a series of popular datasets demonstrate the effectiveness of the proposed FB-Better. Our code has been released at https://github.com/jiaxiaojunQAQ/FP-Better.

==> fig/framework.tex <==
\begin{figure*}[t]
\begin{center}
 \includegraphics[width=0.8\linewidth]{img/Framework.pdf}
\end{center}
\vspace{-3mm}
  \caption{Pipeline of the proposed FGSM-DSD .}
\label{fig:Pipeline}
\vspace{-3mm}
\end{figure*}

==> fig/home.tex <==
\begin{figure}[t]
\begin{center}
 \includegraphics[width=1.0\linewidth]{img/time_acc.pdf}
\end{center}
\vspace{-3mm}
  \caption{ PGD-10 robust accuracy and training time of different FAT methods with ResNet18 as the backbone on the CIFAR-10 dateset. $x$-axis denotes training time (lower is more efficient) and $y$-axis denotes PGD-10 accuracy (higher is more robust).  }
\label{fig:time_acc}
\vspace{-3mm}
\end{figure}

==> latex/method.tex <==
\section{The Proposed Approach}
In this section, we review catastrophic overfitting in Sec.\ref{catastrophic overfitting}  then explore the impact of SD on
single-step AT methods in Sec.\ref{impact of SD}. Moreover, we  propose
a simple yet effective dynamic stochastic depth for FGSM-AT (FGSM-DSD) to further improve the model robustness and training efficiency in Sec.\ref{FGSM-DSD}.




\input{fig/overfitting}
\subsection{Reviewing  catastrophic overfitting}
\label{catastrophic overfitting} 
Catastrophic overfitting which leads to the failure of FGSM-AT~\cite{szegedy2013intriguing} is first noticed by \citet{wong2020fast}. It refers to a phenomenon that during the trianing of single-step AT, the robustness accuracy against multi-step attack methods (such as PGD) suddenly decreases to 0\% after a few epochs. Then \citet{wong2020fast} indicate that FGSM-AT combined with random initialization (FGSM-RS) can prevent catastrophic overfitting.
Several works \cite{andriushchenko2020understanding,kim2020understanding} study and analyze the phenomenon of catastrophic overfitting and find that only using random initialization delayes catastrophic overfitting instead of preventing it. In other word, if the FGSM-RS continues to be trained for a long time, it also encounters catastrophic overftting. As revealed in \cite{andriushchenko2020understanding, kim2020understanding}, FGSM-RS adopt cyclic learning rates~\cite{smith2017cyclical} which can be regrades as an early stopping technology to prevent catastrophic overfitting. Therefore, catastrophic overfitting is not fundamentally solved by FGSM-RS. 
\par To overcome the overfitting,  \citet{andriushchenko2020understanding} and \citet{ kim2020understanding} propose their own methods to prevent catastrophic overfitting from a different perspective. In detail, \citet{andriushchenko2020understanding} propose to adopt a gradient regularization method to prevent the overfitting, called FGSM-GA. While \citet{kim2020understanding} propose a simple yet effective method to adjust the attack step size for FGSM-AT during the training, called FGSM-CKPT. It also can be regarded as a regularization method about the attack step size. As shown in Fig~\ref{fig:ovrrfitting}, it can be observed that compared with FGSM-RS, FGSM-GA and FGSM-CKPT can solve the overfitting problem more efficiently. However, they require more calculating time to preform their regularization methods. Specifically, FGSM-GA needs more calculating time to calculate model gradients to achieve regularization. FGSM-CKPT needs more calculating time to perform forwarding propagation to select the optimal attack step size for the generation of AEs.




\input{table/uniform}
\input{table/Linear}
\subsection{The impact of SD on
single-step AT}
\label{impact of SD} 
In this section, we adopt the partial layers of the model to generate AEs and train them on the generated AEs. In detail, we multiply a random Bernoulli variable $\beta_{\ell}$ which can be regard as a mask and each block in the residual network. During each training iteration, the mask is re-sampled and we can obtain different subnetworks which are composed of  residual blocks with $\beta_{\ell}=1$. Then we adopt FGSM on the subnetwork to generate AEs to conduct adversarial training for the subnetwork. It can be defined as:
\begin{equation}
\min _{\boldsymbol{\theta}} \mathbb{E}_{(\mathbf{x}, {y}) \sim \mathcal{D}}[\max _{\boldsymbol{\delta}_{adv} \in \Omega} \mathcal{L}(\mathbf{x}+\boldsymbol{\delta}_{adv}, {y}, \boldsymbol{\beta};\boldsymbol{\theta}))],
\end{equation}
The adversarial perturbation $\boldsymbol{\delta}_{adv}$ is the core to improve
the model robustness. In this work, it is generated by single-step attack methods (FGSM) on the subnetwork which is composed of residual blocks with $\beta_{\ell}=1$.
It can be defined as:
\begin{equation}
\boldsymbol{\delta}_{adv}=\Pi_{[-\epsilon, \epsilon]}\left[\varphi+\alpha \cdot \operatorname{sign}\left(\nabla_{\mathbf{x}} \mathcal{L}(\mathbf{x}+\varphi, y, \boldsymbol{\beta}; \boldsymbol{\theta})\right)\right],
\label{eq:FGSM_SD}
\end{equation}
where $\boldsymbol{\beta}=\left({\beta}_{\ell}\right)_{0 \leq \ell \leq L}$ is a vector of Bernoulli variables with survival probability parameters $\boldsymbol{p}=\left(p_{\ell}\right)_{1 \leq \ell \leq L}$. Then generated AEs are used to train the subnetwork with the same mask. After each iteration of the adversarial training, the mask is re-sampled. Compare with the adversarial perturbation (Eq.~\ref{eq:FGSM_RS}) used in FGSM-RS, the above adversarial perturbation (Eq.~\ref{eq:FGSM_SD}) depends not only on the model parameters ($\boldsymbol{\theta}$) but also on the mask parameters ($\boldsymbol{\beta}$). Following \cite{huang2016deep}, we explore the impact of two alternative survival probability strategies, \textit{i.e.,} the
uniform and linear strategies, on the FGSM-AT combined with SD, dubbed FGSM-SD. In detail, we perform FGSM-SD with above two alternative strategies of different survival probabilities on CIFAR-10 dataset. The training and evaluation details are presented in Sec.~\ref{Experiments}. As for the uniform strategy, the result is shown in Table~\ref{table:FGSM_SD_uniform}. It can be observed that when $p_{\ell} \leq 0.9 $, the clean and robustness performance improves with the increase of the $p_{\ell}$ value, and similarly, the computation time increases with the increase of the $p_{\ell}$ value. However, when $p_{\ell}=1$, it consumes the most time without achieving excellent performance.  As for the linear strategy, we observed the same experimental phenomenon. 
It indicates that randomly dropping some layers in one-step adversarial training is beneficial to improve model robustness. Moreover, randomly dropping some layers can can further improve the training efficiency of AT. Specifically,  using stochastic depth to conduct AT, we adopt $\widetilde{L}$ to represent the  number of effective residual blocks of the network. It can be defined as:
\begin{equation}
E(\widetilde{L})=\sum_{\ell=1}^{L} p_{\ell},
\end{equation}
where $L$ represents the number of whole residual blocks. Under the linear strategy with $p_{\ell}=0.5$, the expected number of effective residual blocks is equal to $L/2$. In this way, the training time is half of the training time of FGSM-RS.


\input{algo/FGSM_DSD}
\subsection{FGSM-AT with dynamic stochastic depth}
\label{FGSM-DSD} 
 Combined with SD, FGSM-RS not only improves the robustness performance but also further improves the training efficiency. However, as for the FGSM-SD, there is an efficiency-performance trade-off, \textit{i.e.,} the more training time it takes, the more robust the model is. We can understand this phenomenon in terms of the bias-variance trade-off principle\cite{yang2020rethinking,hayou2021regularization}. When $\widetilde{L} / L \rightarrow 0$, the model bias increases (and the model variance decreases). The increase of the bias inevitably deteriorates the model robustness performance. In other words, reducing the training time of FGSM-SD can decrease the model robustness. Moreover, The variance and bias of the model changes dynamically as training progresses. During the whole training stage, using SD with the fixed survival probability $p_{\ell}$ limits the performance improvement
 \par To further improve the model robustness and training efficiency, we propose a dynamically changing survival rate used in SD to conduct adversarial training, called FGSM-DSD. In detail, at the beginning of training, we adopt the subnetwork with the shallow depth (small survival rate $p_{\ell}$ to conduct adversarial training. As the training continues, we gradually improve the survival rate, that is, gradually increase the depth of the model. In this way, the proposed method not only further improves the robustness of the model but also further reduces the computation time. The core of the proposed method is when to adjust the survival rate. We design a sample yet effective adjusting criterion according to the cumulative adversarial training loss over a certain period of time. It can be defined as:  
 \begin{equation}
c(\text{SD})=\sum_{i=1}^{N}\mathcal{L}_{\text{cur}}(\mathrm{x}_{i}, y_{i}, \boldsymbol{\beta}_{i} ; \boldsymbol{\theta}_{i}^{\text{cur}})-\sum_{\ell=1}^{N}\mathcal{L}_{\text{pre}}(\mathrm{x}_{i}, y_{i}, \boldsymbol{\beta}_{i} ; \boldsymbol{\theta}_{i}^{\text{pre}}),
\end{equation}
where $N$ represents the iterative training times over a certain period of time, $\mathcal{L}_{\text{cur}}$ represents the cumulative adversarial training loss for the current certain period of time, and $\mathcal{L}_{\text{pre}}$ represents the cumulative adversarial training loss for the previous certain period of time. if $c(\text{SD})>0$, this means that the model with current depth can continue to be trained to improve robustness performance. Otherwise the model with current depth may have achieved the upper limit of robustness performance. The depth of the current model need to be increased, \textit{i.e.,} increasing the  survival rate $p_{\ell}$. It is can be defined as:
\begin{equation}
p_{\ell}= \begin{cases} p_{\ell}, & , \text { if } c(\text{SD}) \geq 0 ; \\ p_{\ell} + \mu_{\ell} & , \text { otherwise }\end{cases}, \quad 1 \leq \ell \leq L
\end{equation}
where $\mu_{\ell}$ represents the adjusting factor at the $\ell$-th depth of the model. In this work, we combined the proposed method with the linear survival rate strategy to conduct single-step AT. 
The algorithm of FGSM-DSD is summarized in Algorithm ~\ref{alg:FGSM_DSD}.
%  However, during the whole training stage, if we adopt SD with the fixed survival probability $p_{\ell}$ to perform adversarial training, it will limit the performance improvement. In detail, 

\subsection{Generalization analysis}

For our algorithm $\mathcal A$ learns a hypothesis $h$ on the training sample set $S$, the expected risk $\mathcal R(h)$ and empirical risk $\hat{\mathcal R}(h)$ are defined as follows,
\begin{gather*}
	 \mathcal R(h) = \mathbb E_{Z} l(h, Z),~~
	\hat{\mathcal R}_S(h) = \frac{1}{N} \sum_{i=1}^N l(h, z_i).
\end{gather*}
Then, we can obtain a generalization bound of our algorithm based on \citet{he2020robustness}.

\begin{theorem}
\label{thm:high_probability_privacy}
Suppose one employs SGD for adversarial training. $L_{ERM}$ is the maximal gradient norm in ERM. Also, suppose the whole training procedure has $T$ iterations. Then, the algorithm $\mathcal A$ has a high-probability generalization bound as follows. Specifically, the following inequality holds with probability at least $1 - \gamma$:
\begin{align*}
\label{eq:high_probability_privacy}
   & \mathbb{E}\mathcal R(h) - \mathbb{E}\hat{\mathcal R}_S(h) \nonumber\\
   \le & c \left(M(1-e^{-\varepsilon}+e^{-\varepsilon}\delta) \log{N}\log{\frac{N}{\gamma}}+\sqrt{\frac{\log 1 / \gamma}{ N}} \right),
\end{align*}
where
\begin{gather}
	\label{eq:epsilon_whole}
	\varepsilon = \varepsilon_0\sqrt{2 T \log \frac{N}{\delta'}} +T \varepsilon_0 (e^{\varepsilon_0} - 1),~~
	%\label{eq:delta_whole}
	\delta =  \frac{\delta'}{N},\nonumber\\
%	\end{gather*}
%	in which
%	\begin{gather*}
	\label{eq:epsilon_iteration}
	\varepsilon_0= \frac{2 L_{ERM}}{N b} \prod_{i = 1}^d \left( \frac{ \max_{\theta, x, y} \left \| \nabla_{\theta} \mathcal L_{\text{adv}}^i \right \|}{\max_{\theta, x, y} \left \| \nabla_{\text{grad}}^i \right \|} \right),
	\end{gather}
$\nabla_{\theta} \mathcal L_{\text{adv}}^i$ and $\nabla_{\text{grad}}^i$ are the $i$-th entry of $\nabla_{\theta} \mathcal L_{\text{adv}}$ and $\nabla_{\text{grad}}$, respectively, defined for the $i$-th layer, $d$ is the depth, $\delta'$ is a positive real, $\tau$ is the batch size, $I$ is the robustified intensity,
\begin{equation*}
%\label{eq:ri}
I = \frac{ \max_{\theta, x, y} \left \| \nabla_{\theta} \max_{\Vert x^\prime - x \Vert \leq \rho} l (h_{\theta} (x^\prime), y) \right \|}{\max_{\theta, x, y} \left \| \nabla_{\theta} l (h_{\theta} (x), y) \right \|},
\end{equation*}
$b$ is the Laplace parameter, $\gamma$ is an arbitrary probability mass, $M$ is the bound for loss $l$, $N$ is the training sample size, $c$ is a universal constant for any sample distribution,  and the probability is defined over the sample set $S$.
\end{theorem}

The proof is given in Appendix \ref{app:proof}.

\begin{remark}
Eq. (\ref{eq:epsilon_iteration}) characterizes the influence of every layer, where
\begin{equation*}
    \frac{ \max_{\theta, x, y} \left \| \nabla_{\theta} \mathcal L_{\text{adv}}^i \right \|}{\max_{\theta, x, y} \left \| \nabla_{\text{grad}}^i \right \|},
\end{equation*}
characterizes the influence from the $i$-th layer.
\end{remark}

When stochastic depth is employed, some layers are randomly dropped. Thus, the term $\varepsilon_0$ decreases; and therefore, the generalization bound of $\mathbb{E}\mathcal R(h) - \mathbb{E}\hat{\mathcal R}_S(h)$ decreases. This suggests that stochastic depth can improve the generalization.


==> latex/proof.tex <==
\section{ Appendix}
\subsection{Proof for Theorem \ref{thm:high_probability_privacy}}
\label{app:proof}

This appendix gives the proof for Theorem \ref{thm:high_probability_privacy}. The proof is based on \citet{he2020robustness}. We recall some of the paper to make this paper completed.

We first define the following term to measure the intensity of adversarial learning.

\begin{definition}[Robustified Intensity]
\label{def:ri}
For adversarial training, the robustified intensity is defined to be
\begin{equation}
\label{eq:ri}
I = \frac{ \max_{\theta, x, y} \left \| \nabla_{\theta} \max_{\Vert x^\prime - x \Vert \leq \rho} l (h_{\theta} (x^\prime), y) \right \|}{\max_{\theta, x, y} \left \| \nabla_{\theta} l (h_{\theta} (x), y) \right \|},
\end{equation}
where $\| \cdot \|$ is a norm defined in the space of the gradient.
\end{definition}

Empirical study shows that the gradient noise satisfies the Laplacian assumption as follows.

\begin{assumption}
The gradient calculated from a mini-batch is drawn from a Laplacian distribution centered at the empirical risk,
\begin{align*}
\frac{1}{\tau} \sum_{(x, y) \in \mathcal B} \nabla_\theta \max_{\Vert x^\prime - x \Vert \leq \rho} l (h_\theta( x^\prime), y) \sim \mathrm{Lap} \left(\nabla_\theta \hat{\mathcal R}_S^A (\theta), b\right).
\end{align*}
\end{assumption}

Then, we have the following theorem under Laplacian assumption.

\begin{theorem}
\label{thm:privacy_whole}
Suppose one employs SGD for adversarial training. $L_{ERM}$ is the maximal gradient norm in ERM. Also, suppose the whole training procedure has $T$ iterations.
%Suppose all conditions of Theorem \ref{thm:privacy_iteration} hold. 
Then, the adversarial training is $(\varepsilon, \delta)$-differentially private, where
\begin{gather*}
	\label{eq:epsilon_whole}
	\varepsilon = \varepsilon_0\sqrt{2 T \log \frac{N}{\delta'}} +T \varepsilon_0 (e^{\varepsilon_0} - 1),\\
	%\label{eq:delta_whole}
	\delta =  \frac{\delta'}{N},~
	\end{gather*}
	in which
	\begin{gather*}
	%\label{eq:epsilon_iteration}
	\varepsilon_0= \frac{2 L_{ERM}}{N b} I,
	\end{gather*}
and $\delta'$ is a positive real, $\tau$ is the batch size, $I$ is the robustified intensity, and $b$ is the Laplace parameter.
\end{theorem}

Recall the following theorem from \citet{he2020robustness}.

\begin{theorem}[High-Probability Generalization Bound via Differential Privacy]
\label{thm:high_probability_privacy}
Suppose all conditions of Theorem \ref{thm:privacy_whole} hold. Then, the algorithm $\mathcal A$ has a high-probability generalization bound as follows. Specifically, the following inequality holds with probability at least $1 - \gamma$:
\begin{align}
\label{eq:high_probability_privacy}
   & \mathbb{E}_{\mathcal{A}}\mathcal R(\mathcal{A}(S)) - \mathbb{E}_{\mathcal{A}}\hat{\mathcal R}_S(\mathcal{A}(S)) \nonumber\\
   \le & c \left(M(1-e^{-\varepsilon}+e^{-\varepsilon}\delta) \log{N}\log{\frac{N}{\gamma}}+\sqrt{\frac{\log 1 / \gamma}{ N}} \right),
\end{align}
where $\gamma$ is an arbitrary probability mass, $M$ is the bound for loss $l$, $N$ is the training sample size, $c$ is a universal constant for any sample distribution,  and the probability is defined over the sample set $S$.
\end{theorem}

Then, we may prove Theorem \ref{eq:high_probability_privacy}.


\subsection{Experiments on More datasets}
\label{app:Experiments}
\par \noindent \textbf{Results on Tiny ImageNet.} 
The The comparison results of Tiny ImageNet are shown in Table~\ref{table:Tiny_Imagnet}. It can be observed that similar to the results on CIFAR-100 and CIFAR-10, compared with competing single-step AT 
methods, our FP-Better has higher robust accuracy and training efficiency. Besides,  compared with the advanced PGD-2-AT, the proposed FP-Better also achieves better model robustness. For example, under the strong attack (AA), PGD-2-AT achieves performance of about 14\% and 10\% robustness accuracy at the best and last checkpoints, but the proposed FP-Better  achieves
the performance of about 16\% and 15\% robustness accuracy, respectively. More importantly, the proposed FP-Better is about 1.7 times faster than PGD-2-AT.


\input{table/Tiny_imagenet}
\par \noindent \textbf{Results on ImageNet.} 
Following ~\cite{shafahi2019adversarial,wong2020fast}, we set the the maximum perturbation
strength $\epsilon$ to 2, 4, and 8 to conduct comparison experiments with ResNet50.
The The comparison results of Tiny ImageNet are shown in Table~\ref{table:Imagnet}. we can observe that when $\epsilon=2$, all AT methods can achieve the same model robustness. They achieve the performance of about 48\%  robustness accuracy against PGD-10 and PGD-50 attacks. However when the maximum perturbation
strength becomes larger, the proposed FP-Better can achieve the better model robustness against PGD attack. In detail, when $\epsilon=8$, Free-AT achieves
about 19\% and 12\% robustness accuracy under the PGD-10 and PGD-50 attacks. But our FP-Better achieves about 21\% and 13\% robustness accuracy. More importantly, our FP-Better can be 3.2 times faster than Free-AT.




\input{table/Imagenet}

==> table/Linear.tex <==
\begin{table*}[]

\centering

\scalebox{0.8}{

\begin{tabular}{@{}c|cc|cc|cc|cc|cc|cc@{}}
\toprule
\multirow{2}{*}{$p_{\ell}$} & \multicolumn{2}{c|}{1.0}           & \multicolumn{2}{c|}{0.9}                             & \multicolumn{2}{c|}{0.8}           & \multicolumn{2}{c|}{0.7}           & \multicolumn{2}{c|}{0.6}           & \multicolumn{2}{c}{0.5}           \\ \cmidrule(l){2-13} 
                   & \multicolumn{1}{c|}{Best}  & Last  & \multicolumn{1}{c|}{Best}           & Last           & \multicolumn{1}{c|}{Best}  & Last  & \multicolumn{1}{c|}{Best}  & Last  & \multicolumn{1}{c|}{Best}  & Last  & \multicolumn{1}{c|}{Best}  & Last  \\ \midrule \midrule
Clean              & \multicolumn{1}{c|}{73.81} & 83.82 & \multicolumn{1}{c|}{82.96}          & \textbf{85.12} & \multicolumn{1}{c|}{83.84} & 84.03 & \multicolumn{1}{c|}{82.7}  & 83.14 & \multicolumn{1}{c|}{79.47} & 81.88 & \multicolumn{1}{c|}{78.22} & 80.42 \\ \midrule 
PGD-50             & \multicolumn{1}{c|}{41.26} & 0.00  & \multicolumn{1}{c|}{\textbf{48.33}} & 47.88          & \multicolumn{1}{c|}{46.73} & 46.34 & \multicolumn{1}{c|}{46.66} & 45.91 & \multicolumn{1}{c|}{45.66} & 44.58 & \multicolumn{1}{c|}{44.02} & 43.18 \\ \midrule
AA                 & \multicolumn{1}{c|}{37.07} & 0.00  & \multicolumn{1}{c|}{\textbf{44.33}} & 43.84          & \multicolumn{1}{c|}{43.85} & 43.55 & \multicolumn{1}{c|}{43.34} & 42.93 & \multicolumn{1}{c|}{42.57} & 41.97 & \multicolumn{1}{c|}{41.39} & 40.64 \\ \midrule
Time(min)          & \multicolumn{2}{c|}{51}            & \multicolumn{2}{c|}{49}                              & \multicolumn{2}{c|}{47}            & \multicolumn{2}{c|}{45}            & \multicolumn{2}{c|}{43}            & \multicolumn{2}{c}{41}            \\ \bottomrule
\end{tabular}
}
\vspace{-2mm}
\caption{Comparisons of the linear strategy with different survival probabilities. It includes clean and robust accuracy (\%) and training time (minute)  on the  CIFAR-10 dataset. Number in bold indicates the best.
% Number in bold indicates the best of the fast AT methods. 
}
\label{table:FGSM_SD_linear}
\end{table*}
\vspace{-2mm}

==> table/YOPO.tex <==
\begin{table}[t]
\centering
\caption{
Comparison results with YOPO of training time (minute), clean accuracy (\%) and robust accuracy (\%) using ResNet18 on CIFAR-10 database under $\ell_{\infty}= 8/225$. Comparison results are reported in \cite{zhang2019you}. Number in bold indicates the best
}
\label{table:YOPO}
\footnotesize
\setlength\tabcolsep{0.6cm}
\begin{tabular}{@{}cccc@{}}
\toprule
Method            & Clean                      & PGD-20                     & Time(s)                 \\ \midrule
\multicolumn{1}{c}{YOPO-3-5~\cite{zhang2019you}} & \multicolumn{1}{c}{82.14} & \multicolumn{1}{c}{38.18} & \multicolumn{1}{c}{40} \\ \midrule
\multicolumn{1}{c}{YOPO-5-3~\cite{zhang2019you}} & \multicolumn{1}{c}{83.99} & \multicolumn{1}{c}{44.72} & \multicolumn{1}{c}{63} \\ \midrule \midrule
FB-Better (ours)               & \textbf{84.06}             & \textbf{47.96}             &\multicolumn{1}{c}{24}              \\ \bottomrule
\end{tabular}
\end{table}


==> table/uniform.tex <==
\begin{table*}[]

\centering

\scalebox{0.8}{

\begin{tabular}{@{}c|cc|cc|cc|cc|cc|cc@{}}
\toprule
\multirow{2}{*}{$p_{\ell}$} & \multicolumn{2}{c|}{1.0}           & \multicolumn{2}{c|}{0.9}                             & \multicolumn{2}{c|}{0.8}           & \multicolumn{2}{c|}{0.7}           & \multicolumn{2}{c|}{0.6}           & \multicolumn{2}{c}{0.5}           \\ \cmidrule(l){2-13} 
                  & \multicolumn{1}{c|}{Best}  & Last  & \multicolumn{1}{c|}{Best}           & Last           & \multicolumn{1}{c|}{Best}  & Last  & \multicolumn{1}{c|}{Best}  & Last  & \multicolumn{1}{c|}{Best}  & Last  & \multicolumn{1}{c|}{Best}  & Last  \\ \midrule  \midrule
Clean             & \multicolumn{1}{c|}{73.81} & 83.82 & \multicolumn{1}{c|}{\textbf{84.35}} & \textbf{84.35} & \multicolumn{1}{c|}{82.77} & 82.77 & \multicolumn{1}{c|}{80.19} & 80.19 & \multicolumn{1}{c|}{76.98} & 76.98 & \multicolumn{1}{c|}{69.47} & 69.47 \\ \midrule
PGD-50            & \multicolumn{1}{c|}{41.26} & 0.00  & \multicolumn{1}{c|}{\textbf{47.48}} & \textbf{47.48} & \multicolumn{1}{c|}{45.43} & 45.43 & \multicolumn{1}{c|}{41.13} & 41.13 & \multicolumn{1}{c|}{36.12} & 36.12 & \multicolumn{1}{c|}{28.28} & 28.28 \\ \midrule
AA                & \multicolumn{1}{c|}{37.07} & 0.00  & \multicolumn{1}{c|}{\textbf{43.52}} & \textbf{43.52} & \multicolumn{1}{c|}{42.54} & 42.54 & \multicolumn{1}{c|}{38.26} & 38.26 & \multicolumn{1}{c|}{33.58} & 33.58 & \multicolumn{1}{c|}{25.72} & 25.72 \\ \midrule
Time(min)         & \multicolumn{2}{c|}{51}            & \multicolumn{2}{c|}{47}                              & \multicolumn{2}{c|}{41}            & \multicolumn{2}{c|}{37}            & \multicolumn{2}{c|}{32}            & \multicolumn{2}{c}{27}            \\ \bottomrule
\end{tabular}
}
\vspace{-2mm}
\caption{Comparisons of the uniform strategy with different survival probabilities. It includes clean and robust accuracy (\%) and training time (minute)  on the  CIFAR-10 dataset. Number in bold indicates the best.
% Number in bold indicates the best of the fast AT methods. 
}
\label{table:FGSM_SD_uniform}
\end{table*}
\vspace{-2mm}
